Homomorphisms between pure mapping class groups

Let $S$ and $S'$ be orientable finite-type surfaces of genus $g\geq 4$ and $g'$, respectively. We prove that every multitwist-preserving map between pure mapping class groups $\text{PMap}(S)\to \text{PMap}(S')$ is induced by a multi-embedding. As an application, we classify all homomorphisms $\text{PMap}(S)\to \text{PMap}(S')$ for $g\geq 4$ and $g' \leq 6\cdot 2^{g-4}$.

==> contenido/giros.tex <==
El objetivo fundamental de esta sección es probar que 

\rdp{Se puede mejorar a g>=3 ?}
\begin{theorem}
	Sean $S, S'$ dos superficies orientables de tipo finito con géneros $g\geq 4$ y $g'$.  Todo homomorfismo $\varphi: \pmcg(S)\to \pmcg(S')$ que preserva giros es inducido por un embebimiento. 
\end{theorem}

Creo que aquí no tenemos que hacer otra cosa que repetir los argumentos de Aramayona-Souto con pequeñas mejoras técnicas. 

Si $\varphi$ es un homomorfismo que preserva giros, está claro que manda giros (no separantes) en curvas disjuntas a potencias de giros en curvas disjuntas. La primera propiedad que deduciremos será que $\varphi$ manda giros no separantes en giros no separantes y giros que se intersecan una vez en giros que se intersecan una vez. En particular, $\varphi$ manda giros no separantes en giros no separantes. 


\begin{lemma}\label{lemCompartirCompsEsReducible}
  Sean $S,S'$ superficies orientables de tipo finito, donde $S$ tiene género $g\geq1$. Si $\varphi:\pmcg(S) \to \pmcg(S')$ es un homomorfismo que preserva giros, entonces la imagen de un giro no separante es un giro no separante o el inverso de un giro no separante.  Además, $\varphi$ manda giros que se intersecan una vez en giros que se intersecan una vez. 
\end{lemma}
\begin{proof}
  Sean $a,b$ dos curvas en $S$ con $i(a,\,b)=1$. Sabemos que $\varphi(\delta_a) = \delta_{\varphi\cdot a}^n$ para cierto $n\in \mathbb{Z}$. Tenemos que ver que $n=\pm1$ y que la curva $\varphi\cdot a$ es no separante. 

  Como $\varphi$ es no trivial, sabemos que $\varphi(\delta_a) \ne \varphi(\delta_b)$. Por otra parte, sabemos que $\varphi(\delta_a), \varphi(\delta_b)$ son dos multigiros trenzados. Usando la clasificación de multigiros trenzados de deducimos que $i(\varphi\cdot a,\,\varphi\cdot b)=1$ y $n=\pm 1$. 
\end{proof}


\subsection{Reduciendo al caso irreducible}

Un homomorfismo $\homomorfismo$ es \emph{reducible} si existe una multicurva $\eta$ en $S'$ tal que $\varphi(\pmcg(S))$ fija $\eta$ como conjunto. Por su parte, diremos que $\eta$ es una \emph{multicurva reductora} (con respecto a $\varphi$). Un homomorfismo $\varphi$ es \emph{fuertemente reducible} si es reducible y toda multicurva reductora se fija componente a componente. 

\rdp{Es posible que este lema vaya a funcionar incluso si todavía tienes raíces. Esto es, si la imagen de un dehn es un multigiro con raíz, creo el mismo argumento sigue funcionando. }
\begin{lemma}
    Sean $S, S'$ superficies orientables de tipo finito, con $S$ de género $g\geq 1$. Sea $\homomorfismo$ un homomorfismo que preserva giros. Si $\varphi$ es reducible, entonces es fuertemente reducible. 
\end{lemma}
\begin{proof}
    Supongamos que no es fuertemente reducible. Entonces existe una multicurva reductora $\eta =\{\eta_1,\dots ,\,\eta_k\}$ tal que $\varphi(\pmcg(S))$ fija $\eta$ como conjunto pero no fija $\eta$ componente a componente. 

    Como $\varphi(\pmcg(S))$ no fija $\eta$ componente a componente, existe $\eta_i \in \eta$ y una curva no separante $c$ tal que $\varphi(\delta_c) \cdot \eta_i \ne \eta_i$.  Ojo! Aquí estamos usando que $\pmcg(S)$ está generado por giros no separantes, que se sigue de la condición $g\geq 1$. 

    Volviendo a la prueba, tenemos que $\varphi(\delta_c) \cdot \eta_i \ne \eta_i$. Recordemos que $\varphi(\delta_c)=\delta_{\varphi\cdot c}^\epsilon$ con $\epsilon =\pm 1$. Como  $\delta_{\varphi\cdot c}^\epsilon$ no fija $\eta_i$, se sigue que $\varphi\cdot c$ es una curva que interseca a $\eta_i$. 

    Ahora, $\delta_{\varphi\cdot c}^\epsilon\cdot \eta = \eta$. Luego, hay un $m\in \mathbb{N}_{>0}$ tal que $\delta_{\varphi\cdot c}^{\epsilon\cdot m}\cdot \eta_i = \eta_i$. Pero esto es imposible porque $\eta_i$ interseca $\varphi\cdot c$.
    \rdp{ala... como me explayo. Escribir todo en un artículo siempre lo hace más ilegible.}
\end{proof}

Sea $\homomorfismo$ un homomorfismo que preserva giros. Si $\varphi$ es reducible, podemos elegir una multicurva reductora maximal $\eta$ y reducir el homomorfismo cortando por las componentes de $\eta$. El nuevo homomorfismo $\widetilde{\varphi}$ preserva giros y es irreducible.  El objetivo es probar que si $\widetilde{\varphi}$ está inducido por un embebimiento, entonces $\varphi$ también está inducido por un embebimiento. 




==> contenido/multigiros.tex <==

Ahora, utilizamos los resultados de la Sección \ref{subsecGiros} para probar que todo homomorfismo que preserva multigiros está inducido por varios embebimientos. 

La primera observación que tenemos es que si el homomorfismo manda un giro en un multigiro (que no es giro), entonces es reducible. 

\begin{lemma}
	Sea $\varphi:\pmcg(S)\to \pmcg(S')$ un homomorfismo que preserva multigiros, donde $S$ es una superficie de de género $g\geq 3$.  Si $\varphi(\delta_c)$ tiene más de una componente (para $c$ no separante),  entonces $\varphi$ es reducible.
\end{lemma}
\begin{proof}
	Es fácil usar la caracterización de trenzas para encontrar un entorno de la imagen de un conjunto generador de Humphrey (un buen dibujo aclara todo esto). Como estas curvas viven dentro de una superficie, se sigue que $\varphi(\delta_c)$ con más de una componente implica que $\varphi$ es reducible.
\end{proof}

Ahora, cortamos por una multicurva maximal que reduzca $\varphi$ y podemos usar el Teorema [FALTA]  para caracterizar la proyección. Concretamente, sea $\eta$ una multicurva maximal que reduzca $\varphi$. Como $\eta$ reduce $\varphi$ entonces la imagen fija cada curva en $\eta$. Además, como $S$ tiene género $g\geq 3$ (que equivale a pedir $\pmcg(S)^{\text{ab}}=1$) entonces $\varphi(\pmcg(S))$  fija los lados de cada curvas, esto es, $\varphi(\pmcg(S))< \mathcal{Z}_0(\mathbb{T_\eta})$ \rdp{Hay que definir este grupo en algún momento}.  Por tanto, podemos considerar la composición
\[  
\pmcg(S) \xrightarrow{\varphi}\mathcal{Z}_0(\mathbb{T}_\eta) \xrightarrow{\mathcal{C}_\eta}   \prod_i \pmcg(S'_i),
\]
donde los $S'_i$ son las subsuperficies de $S$ que surgen de cortar por la curva maximal $\eta$. Nótese que todas las proyecciones $\varphi_i = \pi_i \circ \mathcal{C}_\eta \circ \varphi$ son irreducibles porque $\eta$ es maximal. Adicionalmente,  $\varphi_i$ es trivial o  manda giros en giros. Por tanto, podemos usar el Teorema [FALTA]  para deducir que $\varphi_i$ es trivial o viene inducida por un embebimiento. 


Solo queda reconstruir $\varphi$ como un homomorfismo inducido por varios embebimientos. Como paso previo, veremos que curvas generadoras no tienen imágense con componentes comunes.

\begin{lemma}
	Sea $\varphi: \pmcg(S)\to \pmcg(S')$ un homomorfismo que preserva multigiros, y $S$ superficie de género $g\geq 3$. Dadas dos curvas generadoras $a,b$ en $S$, los multigiros $\varphi(\delta_a), \varphi(\delta_b)$ no comparten componentes.
\end{lemma}
\begin{proof}
	Si dos curvas generadoras comparten componentes, entonces todos los giros no separantes comparten componentes. Sean $\delta_c, \delta_{c'}$ dos giros no separantes, sabemos que $\mathcal{C}_eta \circ \varphi(\delta_c)$ y $\mathcal{C}_eta \circ \varphi(\delta_{c'})$ no comparten componente porque son inducidos por embebmientos. Luego, las componentes que comparten $\varphi(\delta_c)$ y $\varphi(\delta_{c'})$ son a lo largo de la multicurva $\eta$. 
	
	Dejo como ejercicio al lector usar la condición $g\geq 3$ (hay una linterna no separante!) para comprobar que el multigiro que comparten tiene que ser trivial. 
\end{proof}

Una forma fácil (aunque da un rodeo raro)  de ver que $\varphi$ está inducido por varios embebmientos es la siguiente: 

Considera $\tilde{S}$ la subsuperficie $S$ que cambia cada punto marcado por una componente de frontera (eliminando un entorno abierto del punto marcado). Es bien conocido el mapa $\tilde{S} \xrightarrow{i} S$ y definimos $\tilde{\varphi} = \varphi \circ i$. Obviamente, $\cut_eta \circ \tilde{\varphi}$ está inducido por embebimientos y uno puede construir varios embebimientos que inducen $\tilde{\varphi}$. En este caso, es sencillamente más fácil porque cuando uno tiene fronteras entonces siempre está bien definido el homomorfismo dado por un multiembebimiento. Ahora, nótese que las curvas de las fronteras de $\tilde{\varphi}$ que factorizan por puntos marcados tienen que ser triviales, que es justo la condición para poder construir un multiembebimiento que coincida con $\varphi$ en un conjunto generador. 















==> contenido/prueba_preserva_giros.tex <==
  













==> contenido/raices.tex <==
\subsubsection{Eliminando raíces}
\subsubsection{Describiendo los multigiros}


==> contenido/torsion.tex <==
El primer paso en este tortuoso camino hacia El Teorema es dar condiciones para que un homomorfismo 

\[ \varphi: \pmcg(S)\to \pmcg(S')\]

cumpla que la imagen de un giro tenga orden infinito. 
\rdp{Esta sección ya está completa. Pero no le vendría mal una revisada.}



\begin{proposition}\label{propMatandoTorsion}
    Sean $S$ y $S'$ superficies orientables de género $g\geq 4$ y $g'< 2^g-1$. Si $g=3$, supón $g'<6$. Todo $\varphi$ homomorfismo no trivial 
    \[
    \pmcg(S)\to \pmcg(S'),   
    \]
    envía un giro no separante a un elemento de orden infinito. 
\end{proposition}
\begin{remark}
    En el teorema anterior escribimos $\pmcg(S')$ por elección estética. La demostración que daremos funciona sin cambios para $\mcg(S')$ (solo podemos cambiar el grupo en la imagen!). 
\end{remark}


Esta proposición va a ser un corolario de los dos lemas siguientes. El primer lema lidia con el caso en que mandamos un giro no separante a un elemento de orden dos. En ese caso, la conclusión es más fuerte que la del segundo lema, que trata de cuando el elemento tiene orden finito mayor que dos.

\begin{lemma}\label{lemaGrpSimetrico}
    Sea $S$ una superficie orientable de género $g\geq 3$ y $G$ un grupo. Considere un homomorfismo no trivial
    \[\varphi:\pmcg(S)\to G\]
    que manda un giro no separante a un  elemento de orden dos. Entonces, $G$ contiene  al grupo simétrico en $2g+1$ elementos. 
\end{lemma}
\begin{proof}
    Tomamos $2g+1$ curvas no separantes $c_1, c_2, \dots, c_{2g+1}$ que forman una cadena, i.e, curvas que cumplen $i(c_i, c_j)=1$ si $|i-j|\leq1$ y  $i(c_i,c_j)=0$ si $|i-j| >1$. Considere el el grupo 
    \[
    H = <\delta_{c_1}, \delta_{c_2}\dots,\delta_{c_{2g+1}}>.  
    \]
    Por hipótesis, $\varphi(H) <G$ es un subgrupo generado por elementos $\varphi(\delta_{c_i})$ de orden 2. Más aún, $\varphi(\delta_{c_i})$ y $\varphi(\delta_{c_j})$ o bien cumplen la relación de trenzas si $|i-j|\leq 1$ o bien conmutan si $|i-j|>1$. Se sigue que $\varphi(H)$ es un cociente del grupo simétrico en $2g+1$ elementos. Pero los únicos cocientes son $\{1\},\; \integers/2\integers$ o todo el grupo simétrico. Nótese que $\varphi(H)\not = \{1\}$ porque $\varphi(\delta_{c_i})$ tiene orden dos. También se tiene que $\varphi(H) \ne \integers/2\integers$,  de lo contrario se deduciría $\varphi(\pmcg(S)) =  \integers/2\integers$, que es imposible porque $\pmcg(S)$ tiene abelianización trivial. La única alternativa es que $\varphi(H)<G$ sea el grupo simétrico en $2g+1$ elementos. 
\end{proof}



Ahora, exploramos el caso en que el orden de la imagen es finita mayor que dos. 

\begin{lemma}
    Sea $S$ una superficie orientable de género $g\geq 3$ y $G$ un grupo. Considere un homomorfismo no trivial
    \[\varphi:\pmcg(S)\to G\]
    que manda un giro no separante a un elemento de orden finito mayor que dos, i.e,  $2<d=o(\varphi(\delta_c))<\infty$. Entonces, existe un subgrupo abeliano $V<G$ de orden al menos $m=\min (2\cdot d\cdot n^{g-1},\;d^g)$, donde $n\neq1$ es un divisor de $d$. 

    En particular, si $g>3$  el grupo $V$ tiene orden al menos $2^{g+2}$. Si $g=3$ el grupo $V$ tiene orden al menos $27$.
\end{lemma}
\begin{remark}
    Obsérvese que si $d=2$ el Lema \ref{lemaGrpSimetrico} indica que $G$ contiene un grupo simétrico en $2g+1$ elementos. Por ende, contiene un grupo abeliano de orden $2^{g+1}$.
\end{remark}
\begin{proof}
    Tomamos curvas disjuntas no separantes $a_1,\dots, a_g, a_{g+1}$ tales que $S\setminus \bigcup_{i=1}^g a_i$ sea conexo y $S\setminus \bigcup_{i=2}^{g+1} a_i$ también sea conexo. Vamos a denotar $v_{c}=\varphi(\delta_{c})$ para cualquier curva $c$.

    Sea $n\geq 1$ el natural más pequeño tal que existan valores $k$ y $m_i\in\mathbb{Z}$ con los cuales se satisface la ecuación 
    \[
    v_{a_k}^n = \prod_{i=1, \;i\ne k}^g    v_{a_i}^{m_i}.
    \]
    Sin pérdida de generalidad, vamos a asumir $k=1$. Está claro que $n$ divide a $d$, de lo contrario podríamos encontrar otro natural más pequeño satisfaciendo la igualdad.

    Obsérvese que $n\geq 2$. En efecto, si $n=1$ podemos elegir $h\in \pmcg(S)$ tal que $h\cdot a_1 = a_{g+1}$ y $h\cdot a_i =a_i$  para todo $i\in\{2,\dots,g\}$. Ahora, conjugando 

    \begin{align*}
        v_{a_g} &= \varphi(h)\cdot v_{a_1}\cdot \varphi(h)^{-1} \\ 
        &= \varphi(h)\cdot v_{a_2}^{k_2}\dots v_{a_g}^{k_g}\cdot \varphi(h)^{-1} \\
        &= v_{a_2}^{k_2}\dots v_{a_g}^{k_g} \\ 
        &= v_{a_1}.
    \end{align*}
    Usando que todos los giros no separantes son conjugados, es fácil ver $v_{a_i}=v_{a_j}$ para todo $i,j$. De allí, se seguiría que la imagen de $\varphi$ es cíclica, pero esto obviamente contradice que $\pmcg(S)^{\text{ab}}$ es trivial. Luego, $n\neq 1$.

    Destacamos que $n\geq 2$ y que el mismo argumento de conjugación implica que  cualesquiera dos curvas no separantes $x$ e $y$ satisfacen $v_x^n = v_y^n$. Esta igualdad la guardamos para más adelante. 

    Consideramos el grupo $\tilde{V}=<v_{a_1},\dots,v_{a_g}>$, que es claramente abeliano y finito. Es un ejercicio no muy difícil ver que los elementos en $\tilde{V}$ de la forma
    \[ 
    v_{a_1}^{m_1}\cdot v_{a_2}^{n_2} \dots v_{a_g}^{n_g},  
    \]
    con $m_1\in \integers/d\integers$ y $n_i \in \integers /n\integers$, son todos distintos. Ergo,  el grupo $\tilde{V}$ tiene al menos $d\cdot n^{g-1}$ elementos. Si $n=d$, entonces $\tilde{V} $ tiene al menos $d^g$ elementos y el enunciado se sigue. Queda ver el caso en que $d>n$. 

    Afirmamos que si $d>n$, entonces tiene que existir una curva no separante $c$ contenida en $S\setminus \bigcup_{i=1}^g a_i$  tal que $v_c \not \in \tilde{V}$. Para probarlo, asumimos lo contrario. 

    Supón que toda curva no separante $c$ en $S\setminus \bigcup_{i=1}^g a_i$ cumple que $v_c\in \tilde{V}$. Como $\tilde{V}$ es abeliano, los correspondientes $v_c$ conmutan entre ellos.  Ahora, podemos elegir  curvas no separantes $c_1, c_2, c_3$ y $x$ en $S\setminus \bigcup_{i=1}^g a_i$ tales que $c_1, c_2, c_3$ y $x, a_1, a_2,a_3$ formen una linterna, lo que implica 
    \[
        v_{c_1}v_{c_2} v_{c_3} = v_{x} v_{a_1}v_{a_2}v_{a_3}.
    \]
    La igualdad anterior viene de la relación de linterna en $\pmcg(S)$. Sin embargo, todos los $v_c$ en la igualdad anterior conmutan por la suposición tomada. Ahora, si elevamos la ecuación a la $n$ tenemos  
    \[
        v_{c_1}^n  = v_{x}^n v_{a_1}^nv_{a_2}^nv_{a_3}^nv_{c_2}^{-n} v_{c_3}^{-n} = v_{c_1}^{2n},
    \]
    donde la última igualdad viene de que $v_a^n=v_b^n$ para cualesquiera dos curvas no separantes. Ahora sí! La ecuación anterior nos dice que $v_c^n=1$, pero eso es imposible porque $n<d=o(v_c)$. Hemos partido de una suposición falsa. Por tanto, debe de existir alguna curva no separante $c$ en  $S\setminus \bigcup_{i=1}^g a_i$  con $v_c\not \in \tilde{V}$, fijamos una curva $c$ con esta propiedad. 

    Para terminar con el caso $d>n$, basta con ver que el grupo abeliano $<\tilde{V}, v_c>$  contiene elementos de la forma 
    \[ 
    v_c^{\epsilon}\cdot v_{a_1}^{m_1}\cdot v_{a_2}^{n_2} \dots v_{a_g}^{n_g},  
    \]
    con $\epsilon \in \{0,1\}$, $m_1\in \integers/d\integers$ y $n_i \in \integers /n\integers$, y   todos esos elementos son distintos. En otras palabras, $<\tilde{V}, v_c>$ tiene por lo menos $2\cdot d\cdot n^{g-1}$ elementos.
\end{proof}


Ya estamos preparados para atacar la Proposición \ref{propMatandoTorsion}. 


\begin{proof}[Demostración de la Proposición \ref{propMatandoTorsion}]
    Supongamos lo contrario, que existe un giro no separante $\delta_c$ cuya imagen tiene orden $d<\infty$. 

    Si $d=2$, entonces $\pmcg(S')$ contiene un subgrupo finito de orden $(2g+1)!$. Recordemos que el orden máximo de un subgrupo finito de $\pmcg(S')$ es $84(g'-1)$. Se sigue que $(2g+1)! \leq 84(g'-1)$ y con ello 
    \[
        g'\geq \frac{(2g+1)!}{84}+1 \geq 2^g-1.    
    \]
    Pero esto contradice que $g' < 2^g-1$. Luego, $\varphi(\delta_c)$ tiene orden $d>2$. 

    Si $d>2$ y $g>3$, entonces $\varphi(\pmcg(S))$ contiene un subgrupo abeliano finito de orden $2^{g+2}$. Recordemos que el subgrupo abeliano finito más grande de $\pmcg(S')$ tiene orden $4g'+4$. Por tanto, $2^{g+2}\leq 4g' + 4$ que implica $2^{g} -1 \leq g'$. Pero esto contradice que $g'<2^g-1$. Luego, para $g>3$ y $g'<2^g-1$, el elemento $\varphi(\delta_c)$ tiene orden infinito.

    Por último, si $g=3$ y $d>2$ la imagen de $\varphi$ contiene un subgrupo abeliano finito de orden al menos 27. De nuevo, usando la cota de subgrupos abeliano finitos, tenemos que $27\leq4g'+4$. Ergo, $6\leq g'$. Por tanto, si $g=3$ y $g'<6$ entonces un giro no separante va aun elemento de orden infinito.

\end{proof}

